A Unified Catalog-level Reanalysis of Stage-III Cosmic Shear Surveys

Cosmological parameter constraints from recent galaxy imaging surveys are reaching $2-3\%$-level accuracy. The upcoming Legacy Survey of Space and Time (LSST) of the Vera C. Rubin Observatory will produce sub-percent level measurements of cosmological parameters, providing a milestone test of the $\Lambda$CDM model. To supply guidance to the upcoming LSST analysis, it is important to understand thoroughly the results from different recent galaxy imaging surveys and assess their consistencies. In this work we perform a unified catalog-level reanalysis of three cosmic shear datasets: the first year data from the Dark Energy Survey (DES-Y1), the 1,000 deg$^{2}$ dataset from the Kilo-Degree Survey (KiDS-1000), and the first year data from the Hyper Suprime-Cam Subaru Strategic Program (HSC-Y1). We utilize a pipeline developed and rigorously tested by the LSST Dark Energy Science Collaboration to perform the reanalysis and assess the robustness of the results to analysis choices. We find the $S_{8}$ constraint to be robust to two different small-scale modeling approaches, and varying choices of cosmological priors. Our unified analysis allows the consistency of the surveys to be rigorously tested and we find the three surveys to be statistically consistent. Due to the partially overlapping footprint, we model the cross-covariance between KiDS-1000 and HSC-Y1 approximately when combining all three datasets, resulting in a $1.6-1.9\%$ constraint on $S_8$ given different assumptions on the cross-covariance.

==> authors.tex <==
% Place your name and orcidID in this file in alphabetical order.


\author[Emily P. Longley et al.]{
Emily P. Longley,$^{1}$\thanks{E-mail: mn@ras.org.uk (KTS)}
Chihway Chang,$^{2,3}$
Chris Walter,$^{1}$
Joe Zuntz,$^{4}$
Maria E. S. Pereira,,$^{5}$
Mustapha Ishak,$^{6}$
Rachel Mandelbaum,$^{7}$
Hironao Miyatake,$^{8,9}$
Andrina Nicola,$^{10}$
Eske Pedersen,$^{11}$
Judit Prat,$^{2,3}$
Javier Sanchez,$^{12}$
Tilman Tr{\"o}ster,$^{13}$
Michael Troxel,$^{1}$
Angus Wright,$^{14}$
The LSST Dark Energy Science Collaboration
\\
% List of institutions
$^{1}$Department of Physics, Duke University, Durham NC 27708, USA\\
$^{2}$Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA \\
$^{3}$Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA \\
$^{4}$Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, United Kingdom \\
$^{5}$Hamburger Sternwarte, Universit\"{a}t Hamburg, Gojenbergsweg 112, 21029 Hamburg, Germany \\
$^{6}$Department of Physics, The University of Texas at Dallas, Richardson, TX 75080, USA \\
$^{7}$Department of Physics, Carnegie Mellon University, Pittsburgh, PA 15213, USA \\
$^{8}$Kobayashi-Maskawa Institute for the Origin of Particles and the Universe (KMI),
Nagoya University, Nagoya, 464-8602, Japan \\
$^{9}$Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study (UTIAS), The University of Tokyo, Chiba 277-8583, Japan \\
$^{10}$Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ
08544, USA \\
$^{11}$Department of Physics, Harvard University 17 Oxford street, Cambridge, MA 02138, USA \\
$^{12}$Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA \\
$^{13}$Institute for Astronomy, University of Edinburgh, Royal Observatory, Blackford Hill, Edinburgh, EH9 3HJ, UK \\
$^{14}$Ruhr-University Bochum, Faculty of Physics and Astronomy, Astronomical Institute (AIRUB), German Centre for Cosmological Lensing, 44780 Bochum, Germany

}
